Programming with Timespans in Interactive Visualizations

Modern interactive visualizations are akin to distributed systems, where user interactions, background data processing, remote requests, and streaming data read and modify the interface at the same time. This concurrency is crucial to provide an interactive user experience---forbidding it can cripple responsiveness. However, it is notoriously challenging to program distributed systems, and concurrency can easily lead to ambiguous or confusing interface behaviors. In this paper, we present DIEL, a declarative programming model to help developers reason about and reconcile concurrency-related issues. Using DIEL, developers no longer need to procedurally describe how the interface should update based on different input events, but rather declaratively specify what the state of the interface should be as queries over event history. We show that resolving conflicts from concurrent processes in real-world interactive visualizations can be done in a few lines of DIEL code.

==> content/diagnosis.tex <==
% \section{The Unruly State of the User Interface}
% \label{sec:diagnosis}

% Before proceeding, we introduce two more examples of overlapping timespans for the reader to gain intuition.  We refer back to these examples in later sections.  The examples are based on the tweet visualization in Figure~\ref{fig:tweetVis}.


% Big data analytics applications often have a client-server architecture, where interactions triggers requests to servers, whose response updates the visualization~\cite{stolte2002polaris,liu2013immens, lins2013nanocubes, fekete2015progressivis}.

% \begin{example}
%   The user brushes to select more tweets to filter the other two charts to the right.  As the user is brushing, fine-grained requests are being sent, at a rate of 90ms (throttled).  However, the response delay happen to be around 100ms.  What should the application do when it receives a response for a request from a now outdated brush interaction?
  
%   One option is to block the brush, which makes handling the results easier.  However the user would experience temporary freezes as they are dragging---the brush is stuck in one position and then abruptly move to another. Another option is to preempt the previous requests, and only render the most recent one, in which case only the last result of the brush will update, and the user will not see any intermediate results.  Another option is to render as the results are received, the user will see a continuous update based on their fine-grained brush interaction, with short, hard-to-detect lag.  However, the results may be out of order and introduce inaccurate visual effects.  For instance, an otherwise smooth sequence of values may appear to fluctuate.
%   \label{exp:preempt}
% \end{example}
 


==> content/enhanced.tex <==
\section{Enhanced DIEL}
\label{sec:enhanced}

\yifan{unclear if we need to cut}

\sys's use of SQL allows us to leverage useful features of standard SQL engines such as a \textbf{constraint}s.  Constraints in SQL can check for uniqueness, null values, foreign keys, as well as custom assertions, e.g., \texttt{x > 20}, which are particularly useful for debugging in \sys---they help pinpoint code fragments that break assumptions.  For instance, the \texttt{not null} constraint used in line 2 \jmh{of what!} will throw an exception if the constraint is violated in development mode; in deployment mode, such an input is ignored.  The detection is useful for example, to identify null arguments supplied by a JavaScript \texttt{input} call, which if left unnoticed can cause strange outputs, which may be difficult to debug otherwise since the developer needs to trace which table or query logic is broken.

Constraints can also be used to handle ill-defined interactions.  Much like a transaction in databases, inputs will not be committed to history should any constraints be violated.  For instance, when a brush completes in an undefined region on the screen, the brush will not be persisted in \sys because the bounding box is partially null; as a result the timestep does not advance, and no update will happen.  Out implementation supports constraints for input, output, and views, in addition to tables.

Beyond augmenting the constraints, we provide three other operators useful for programming interactive visualizations in \sys.

Additionally, we provides an abstraction for (3) \textbf{finite state machines} (FSM), which are useful to reason about interactions~\cite{kin2012proton,satyanarayan2014declarative}).  The \texttt{match} operator takes a column from a relation and a regular expression (a way to express FSM) on the value of the column.
For instance, to capture the bounds of a brush with a sequence of \texttt{down},\texttt{move}, \texttt{move}..., \texttt{up}, a developer can use '(down)(?:move)*(up)' to get the start and end of the events in a brush.  The \texttt{?:} syntax is standard regex to skip capturing groups.  Shown in Listings~\ref{lst:match}. \jmh{AWK}
The return value of a \texttt{match} query is also a relation, which contains the selected columns of matching rows, with an additional column that identifies the matching group (\texttt{mg}).

\begin{listing}[h]
  \begin{minted}{sql}
-- returns e.g., (0, 1, 'down'), (0, 10, 'up')
select mg, x, mouseEvent from brushItx
  match mouseEvent on '(down)(?:move)*(up)';
  \end{minted}
  \caption{Example use of the \texttt{match} operator}
  \label{lst:match}
\end{listing}
